Selecting Diverse Models for Scientific Insight

Model selection often aims to choose a single model, assuming that the form of the model is correct. However, there may be multiple possible underlying explanatory patterns in a set of predictors that could explain a response. Model selection without regard for model uncertainty can fail to bring these patterns to light. We explore multi-model penalized regression (MMPR) to acknowledge model uncertainty in the context of penalized regression. We examine how different penalty settings can promote either shrinkage or sparsity of coefficients in separate models. The method is tuned to explicitly limit model similarity. A choice of penalty form that enforces variable selection is applied to predict stacking fault energy (SFE) from steel alloy composition. The aim is to identify multiple models with different subsets of covariates that explain a single type of response.

==> bma_condpostmean.tex <==
% latex table generated in R 3.6.1 by xtable 1.8-4 package
% Wed Apr 29 19:50:36 2020
\begin{table}[ht]
\centering
\caption{BMA conditional posterior mean of coefficients for covariates in simulations} 
\label{tab:bma_coeffs}
\begin{tabular}{|c|cccccc|}
  \hline
 & x1 & x2 & x3 & x4 & x5 & x6 \\ 
  \hline
Case 1 & 8.88 & 15.28 & 10.40 & -3.18 & 2.27 & -0.90 \\ 
  Case 2 & 3.53 & 12.62 & 9.27 & -0.16 & -2.76 & -2.66 \\ 
  Case 3 & 23.56 & 14.34 & 8.18 & 5.12 & 3.72 & 2.04 \\ 
  Case 4 & 6.50 & 17.20 & 13.77 & 0.94 & 3.57 & 1.03 \\ 
  Case 5 & 6.28 & 14.69 & 19.54 & -1.40 & -0.96 & -0.27 \\ 
  Case 6 & 7.82 & 15.77 & 6.30 & -0.76 & 9.82 & -5.81 \\ 
  Case 7 & -2.56 & 16.40 & 6.98 & 6.52 & 4.12 & 3.83 \\ 
   \hline
\end{tabular}
\end{table}


==> bma_models.tex <==
% latex table generated in R 3.6.1 by xtable 1.8-4 package
% Fri Jun 12 08:10:08 2020
\begin{table}[ht]
\centering
\caption{BMA maximum likelihood models for Case 4 simulation data} 
\label{tab:bma_models}
\begin{tabular}{|c|cccccc|}
  \hline
 & x1 & x2 & x3 & x4 & x5 & x6 \\ 
  \hline
Model 1 & 6.50 & 16.20 & 12.77 & - & - & - \\ 
  Model 2 & - & 18.37 & 14.93 & - & - & - \\ 
  Model 3 & 6.50 & 16.20 & 12.77 & - & 3.57 & - \\ 
  Model 4 & - & 18.37 & 14.93 & - & 3.57 & - \\ 
  Model 5 & 6.50 & 16.20 & 12.77 & - & - & 1.03 \\ 
  Model 6 & 6.50 & 16.20 & 12.77 & 0.94 & - & - \\ 
  Model 7 & - & 18.37 & 14.93 & - & - & 1.03 \\ 
  Model 8 & - & 18.37 & 14.93 & 0.94 & - & - \\ 
   \hline
\end{tabular}
\end{table}


==> bma_postprob.tex <==
% latex table generated in R 4.0.2 by xtable 1.8-4 package
% Thu Sep 17 11:30:13 2020
\begin{table}[ht]
\centering
\caption{BMA posterior probabilities of covariates in simulations} 
\label{tab:bma_prob}
\begin{tabular}{|c|cccccc|}
  \hline
 & x1 & x2 & x3 & x4 & x5 & x6 \\ 
  \hline
Case 1 & 1.00 & 1.00 & 1.00 & 0.16 & 0.11 & 0.08 \\ 
  Case 2 & 0.11 & 1.00 & 0.89 & 0.06 & 0.09 & 0.09 \\ 
  Case 3 & 0.95 & 0.16 & 0.15 & 0.09 & 0.07 & 0.06 \\ 
  Case 4 & 0.54 & 1.00 & 1.00 & 0.08 & 0.21 & 0.08 \\ 
  Case 5 & 0.13 & 0.43 & 0.83 & 0.07 & 0.06 & 0.06 \\ 
  Case 6 & 0.65 & 1.00 & 0.54 & 0.10 & 0.94 & 0.32 \\ 
  Case 7 & 0.07 & 1.00 & 0.44 & 0.36 & 0.17 & 0.15 \\ 
   \hline
\end{tabular}
\end{table}


==> commands.tex <==
\newcommand{\btheta}{ \mbox{\boldmath $\theta$}}
\newcommand{\bmu}{ \mbox{\boldmath $\mu$}}
\newcommand{\balpha}{ \mbox{\boldmath $\alpha$}}
\newcommand{\bbeta}{ \mbox{\boldmath $\beta$}}
\newcommand{\bmeta}{ \mbox{\boldmath $\eta$}}

\newcommand{\bdelta}{ \mbox{\boldmath $\delta$}}
\newcommand{\blambda}{ \mbox{\boldmath $\lambda$}}
\newcommand{\bgamma}{ \mbox{\boldmath $\gamma$}}
\newcommand{\brho}{ \mbox{\boldmath $\rho$}}
\newcommand{\bpsi}{ \mbox{\boldmath $\psi$}}
\newcommand{\bepsilon}{ \mbox{\boldmath $\epsilon$}}
\newcommand{\bomega}{ \mbox{\boldmath $\omega$}}
\newcommand{\bDelta}{ \mbox{\boldmath $\Delta$}}
\newcommand{\bSigma}{ \mbox{\boldmath $\Sigma$}}
\newcommand{\bOmega}{ \mbox{\boldmath $\Omega$}}
\newcommand{\bGamma}{ \mbox{\boldmath $\Gamma$}}
\newcommand{\bA}{ \mbox{\bf A}}
\newcommand{\ba}{ \mbox{\bf a}}
\newcommand{\be}{ \mbox{\bf e}}
\newcommand{\bP}{ \mbox{\bf P}}
\newcommand{\bx}{ \mbox{\bf x}}
\newcommand{\bX}{ \mbox{\bf X}}
\newcommand{\bB}{ \mbox{\bf B}}
\newcommand{\bZ}{ \mbox{\bf Z}}
\newcommand{\by}{ \mbox{\bf y}}
\newcommand{\bY}{ \mbox{\bf Y}}
\newcommand{\bz}{ \mbox{\bf z}}
\newcommand{\bh}{ \mbox{\bf h}}
\newcommand{\bmm}{ \mbox{\bf m}}
\newcommand{\br}{ \mbox{\bf r}}
\newcommand{\bt}{ \mbox{\bf t}}
\newcommand{\bs}{ \mbox{\bf s}}
\newcommand{\bb}{ \mbox{\bf b}}
\newcommand{\bff}{ \mbox{\bf f}}
\newcommand{\bL}{ \mbox{\bf L}}
\newcommand{\bu}{ \mbox{\bf u}}
\newcommand{\bv}{ \mbox{\bf v}}
\newcommand{\bV}{ \mbox{\bf V}}
\newcommand{\bG}{ \mbox{\bf G}}
\newcommand{\bC}{ \mbox{\bf C}}
\newcommand{\bg}{ \mbox{\bf g}}
\newcommand{\bH}{ \mbox{\bf H}}
\newcommand{\bI}{ \mbox{\bf I}}
\newcommand{\bD}{ \mbox{\bf D}}
\newcommand{\bM}{ \mbox{\bf M}}
\newcommand{\bW}{ \mbox{\bf W}}
\newcommand{\bw}{ \mbox{\bf w}}
\newcommand{\bT}{ \mbox{\bf T}}
\newcommand{\bQ}{ \mbox{\bf Q}}
\newcommand{\bR}{ \mbox{\bf R}}
\newcommand{\bfe}{ \mbox{\bf e}}
\newcommand{\bzero}{ \mbox{\bf 0}}
\newcommand{\iid}{\stackrel{iid}{\sim}}
\newcommand{\indep}{\perp\!\!\!\perp}
\newcommand{\Xtil}{{\tilde X}}
\newcommand{\bXtil}{\bf {\tilde X}}

\newcommand{\calR}{{\cal R}}
\newcommand{\calL}{{\cal L}}
\newcommand{\calG}{{\cal G}}
\newcommand{\calD}{{\cal D}}
\newcommand{\calC}{{\cal C}}
\newcommand{\calS}{{\cal S}}
\newcommand{\calB}{{\cal B}}
\newcommand{\calA}{{\cal A}}
\newcommand{\calT}{{\cal T}}
\newcommand{\calO}{{\cal O}}
\newcommand{\calN}{{\cal N}}
\newcommand{\calK}{{\cal K}}
\newcommand{\argmax}{{\mathop{\rm arg\, max}}}
\newcommand{\argmin}{{\mathop{\rm arg\, min}}}
\newcommand{\Frechet}{\mbox{Fr$\acute{\mbox{e}}$chet}}
\newcommand{\Matern}{ \mbox{Mat$\acute{\mbox{e}}$rn}}
\newcommand{\Prob}{\mbox{Prob}}
\newcommand{\FGEV}{F_{\mbox{{\tiny GEV}}}}
\newcommand{\fGEV}{f_{\mbox{{\tiny GEV}}}}
\newcommand{\FMGEV}{F_{\mbox{{\tiny MGEV}}}}
\newcommand{\fMGEV}{f_{\mbox{{\tiny MGEV}}}}
\newcommand{\beq}{ \begin{equation}}
\newcommand{\eeq}{ \end{equation}}
\newcommand{\beqn}{ \begin{eqnarray}}
\newcommand{\eeqn}{ \end{eqnarray}}



==> fs_coef.tex <==
% latex table generated in R 4.0.2 by xtable 1.8-4 package
% Thu Sep 24 12:01:11 2020
\begin{table}[ht]
\centering
\caption{Forward selection coefficient estimates of top M models for simulation data} 
\label{tab:fs_coeffs}
\begin{tabular}{|c|cccccc|}
  \hline
 & x1 & x2 & x3 & x4 & x5 & x6 \\ 
  \hline
 & 10.40 & 8.88 & 15.28 & - & - & - \\ 
  Case 1 & 10.40 & 8.88 & 15.28 & -3.18 & - & - \\ 
    & 10.40 & 8.88 & 15.28 & -3.18 & 2.27 & - \\ 
   \hline
   & 10.40 & 12.32 & 9.16 & - & - & - \\ 
  Case 2 & 9.16 & 3.53 & 10.56 & -3.18 & - & - \\ 
      & 10.40 & 16.90 & 15.28 & -3.18 & 2.27 & - \\ 
   \hline
     & 26.15 & 12.32 & 9.16 & - & - & - \\ 
  Case 3 & 19.53 & 3.53 & 8.18 & -3.18 & - & - \\ 
        & 19.53 & 16.90 & 9.30 & -3.18 & 2.27 & -1.54 \\ 
   \hline
       & 12.77 & 6.50 & 16.20 & - & - & - \\ 
  Case 4 & 19.53 & 18.37 & 14.93 & -3.18 & - & - \\ 
          & 12.77 & 6.50 & 16.20 & -3.18 & 3.57 & -1.54 \\ 
   \hline
         & 12.77 & 6.50 & 23.10 & - & - & - \\ 
  Case 5 & 19.53 & 13.64 & 10.51 & -3.18 & - & - \\ 
            & 12.77 & 13.64 & 10.51 & -1.40 & 3.57 & -1.54 \\ 
   \hline
           & 6.18 & 7.82 & 8.83 & - & 14.40 & - \\ 
  Case 6 & 8.83 & 7.82 & 10.51 & -3.18 & 14.40 & - \\ 
              & 6.18 & 7.82 & 11.74 & -1.40 & 14.40 & -5.81 \\ 
   \hline
             & 6.18 & 16.24 & 7.13 & - & 14.40 & - \\ 
  Case 7 & 8.83 & 16.24 & 10.51 & -3.18 & 14.40 & - \\ 
                    & 6.18 & 16.24 & 7.13 & -1.40 & 4.12 & -5.81 \\ 
   \hline
\end{tabular}
\end{table}


==> lasso_coef.tex <==
% latex table generated in R 3.6.1 by xtable 1.8-4 package
% Wed Apr 29 20:13:24 2020
\begin{table}[ht]
\centering
\caption{LASSO coefficient estimates for simulation data} 
\label{tab:lasso_coeffs}
\begin{tabular}{|c|cccccc|}
  \hline
 & x1 & x2 & x3 & x4 & x5 & x6 \\ 
  \hline
Case 1 & 8.21 & 14.61 & 9.73 & -2.50 & 1.60 & -0.23 \\ 
  Case 2 & 2.93 & 10.26 & 8.94 & 0.02 & -0.99 & -1.17 \\ 
  Case 3 & 17.44 & 2.75 & 6.13 & - & - & - \\ 
  Case 4 & 6.07 & 15.77 & 12.34 & - & 2.71 & - \\ 
  Case 5 & 1.70 & 9.15 & 12.31 & -0.38 & - & - \\ 
  Case 6 & 7.28 & 13.86 & 5.72 & -0.71 & 10.12 & -4.20 \\ 
  Case 7 & - & 15.20 & 4.43 & 1.85 & 3.00 & 0.08 \\ 
   \hline
\end{tabular}
\end{table}


==> mmpr_models.tex <==
% latex table generated in R 3.6.1 by xtable 1.8-4 package
% Fri Jun 12 08:10:29 2020
\begin{table}[ht]
\centering
\caption{MMPR models for Case 4 simulation data} 
\label{tab:mmpr_models}
\begin{tabular}{|c|cccccc|}
  \hline
 & x1 & x2 & x3 & x4 & x5 & x6 \\ 
  \hline
Model 1 & 11.73 & 3.68 & - & - & - & - \\ 
  Model 2 & - & 16.43 & - & - & - & - \\ 
  Model 3 & - & - & 16.70 & - & - & - \\ 
   \hline
\end{tabular}
\end{table}


==> sim_100_cases.tex <==
% latex table generated in R 4.0.2 by xtable 1.8-4 package
% Thu Oct 08 15:48:21 2020
\begin{table}[ht]
\centering
\caption{Mean and standard error coefficients in simulation cases.} 
\label{cases_coef}
\begin{tabular}{|c|c|cccccc|}
  \hline
Case & Model & x1 & x2 & x3 & x4 & x5 & x6 \\ 
  \hline
 & Model 1 & 8.95 (0.13) & 8.91 (0.1) & 8.94 (0.1) & 0.01 (0.1) & 0 (0.14) & -0.02 (0.07) \\ 
  1 & Model 2 & 0 (0) & 0 (0) & 0 (0) & 0 (0) & -0.01 (0.02) & 0 (0) \\ 
   & Model 3 & 0 (0) & 0 (0) & 0 (0) & 0 (0) & 0 (0) & 0 (0) \\ 
   \hline
 & Model 1 & 11.94 (0.07) & 0 (0) & 0.48 (0.04) & 6.07 (0.08) & 0 (0) & -0.01 (0.06) \\ 
  2 & Model 2 & 0 (0) & 17.69 (0.1) & 0 (0) & 0 (0) & 1.68 (0.11) & 0.01 (0.05) \\ 
   & Model 3 & 4.44 (0.04) & 0 (0) & 14.22 (0.1) & 0 (0) & 0 (0) & 0.04 (0.07) \\ 
   \hline
 & Model 1 & 15.73 (0.17) & 0 (0) & 0 (0) & 10.38 (0.17) & 0 (0) & -0.03 (0.11) \\ 
  3 & Model 2 & 0 (0) & 22.91 (0.24) & 0 (0) & 0 (0) & 2.99 (0.23) & -0.05 (0.16) \\ 
   & Model 3 & 7.11 (0.06) & 0 (0) & 18.5 (0.16) & 0 (0) & 0 (0) & -0.01 (0.13) \\ 
   \hline
 & Model 1 & 14.02 (0.21) & 1.94 (0.17) & 1.97 (0.21) & -0.03 (0.05) & 0 (0.05) & 0.05 (0.08) \\ 
  4 & Model 2 & 1.96 (0.11) & 14.02 (0.12) & 1.95 (0.12) & -0.03 (0.08) & 0.01 (0.07) & 0.05 (0.1) \\ 
   & Model 3 & 1.96 (0.04) & 1.96 (0.09) & 14.01 (0.12) & -0.01 (0.07) & 0.02 (0.08) & 0.01 (0.06) \\ 
   \hline
 & Model 1 & 21.31 (0.33) & 3.77 (0.34) & 0 (0) & -0.02 (0.08) & 0.03 (0.05) & 0.02 (0.06) \\ 
  5 & Model 2 & 0 (0) & 21.46 (0.42) & 3.61 (0.43) & 0.01 (0.11) & 0.04 (0.2) & -0.02 (0.15) \\ 
   & Model 3 & 3.65 (0.36) & 0 (0) & 21.43 (0.36) & 0.03 (0.12) & 0.03 (0.07) & -0.03 (0.11) \\ 
   \hline
 & Model 1 & 13.45 (0.09) & 0 (0) & 8.91 (0.09) & 0 (0) & 0.02 (0.07) & 0 (0.08) \\ 
  6 & Model 2 & 0 (0) & 13.43 (0.11) & 0 (0) & 4.45 (0.12) & 0.04 (0.07) & -0.01 (0.03) \\ 
   & Model 3 & 0 (0.01) & 0 (0) & 0 (0) & 0 (0) & 0.01 (0.08) & 0 (0.07) \\ 
   \hline
 & Model 1 & 17.01 (0.1) & 0 (0) & 8.93 (0.11) & 0 (0) & -0.06 (0.27) & 0.04 (0.27) \\ 
  7 & Model 2 & 0 (0) & 17.02 (0.09) & 0 (0) & 8.05 (0.1) & 0 (0.07) & -0.03 (0.07) \\ 
   & Model 3 & 0 (0) & 0 (0) & 0 (0) & 0 (0) & 0 (0.01) & -0.01 (0.03) \\ 
   \hline
\end{tabular}
\end{table}


==> sim_100_nonzero.tex <==
% latex table generated in R 4.0.2 by xtable 1.8-4 package
% Thu Oct 08 15:38:17 2020
\begin{table}[ht]
\centering
\caption{Proportion of nonzero coefficient estimates in each simulation case.} 
\label{nonzero}
\begin{tabular}{|c|c|cccccc|}
  \hline
Case & Model & x1 & x2 & x3 & x4 & x5 & x6 \\ 
  \hline
 & Model 1 & 1.00 & 1.00 & 1.00 & 0.88 & 0.94 & 1.00 \\ 
  1 & Model 2 & 0.00 & 0.00 & 0.00 & 0.12 & 0.06 & 0.00 \\ 
   & Model 3 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 \\ 
   \hline
 & Model 1 & 1.00 & 0.00 & 1.00 & 1.00 & 0.00 & 0.56 \\ 
  2 & Model 2 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.50 \\ 
   & Model 3 & 1.00 & 0.00 & 1.00 & 0.00 & 0.00 & 0.56 \\ 
   \hline
 & Model 1 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.44 \\ 
  3 & Model 2 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.69 \\ 
   & Model 3 & 1.00 & 0.00 & 1.00 & 0.00 & 0.00 & 0.56 \\ 
   \hline
 & Model 1 & 1.00 & 1.00 & 1.00 & 0.50 & 0.50 & 0.56 \\ 
  4 & Model 2 & 1.00 & 1.00 & 1.00 & 0.44 & 0.62 & 0.62 \\ 
   & Model 3 & 1.00 & 1.00 & 1.00 & 0.38 & 0.88 & 0.50 \\ 
   \hline
 & Model 1 & 1.00 & 1.00 & 0.00 & 0.44 & 0.69 & 0.38 \\ 
  5 & Model 2 & 0.00 & 1.00 & 1.00 & 0.50 & 0.81 & 0.69 \\ 
   & Model 3 & 1.00 & 0.00 & 1.00 & 0.56 & 0.62 & 0.31 \\ 
   \hline
 & Model 1 & 1.00 & 0.00 & 1.00 & 0.00 & 0.38 & 0.56 \\ 
  6 & Model 2 & 0.00 & 1.00 & 0.00 & 1.00 & 0.50 & 0.25 \\ 
   & Model 3 & 0.12 & 0.00 & 0.00 & 0.00 & 0.12 & 0.19 \\ 
   \hline
 & Model 1 & 1.00 & 0.00 & 1.00 & 0.00 & 0.69 & 0.38 \\ 
  7 & Model 2 & 0.00 & 1.00 & 0.00 & 1.00 & 0.31 & 0.56 \\ 
   & Model 3 & 0.00 & 0.00 & 0.00 & 0.00 & 0.06 & 0.06 \\ 
   \hline
\end{tabular}
\end{table}

